Massive 2- and 3-loop corrections to hard scattering processes in QCD

With the increasing experimental precision available at colliders, higher-order perturbative calculations are required to reduce the theory uncertainty in order to extract crucial QCD parameters, such as the strong coupling constant, to the required precision, often the order of one percent. For this reason, the contributions of the massive charm and bottom quarks need to be taken into account in hadronic processes such as deep-inelastic scattering. In this thesis, we calculate to order $\alpha_s^3$ the two-mass contributions to the twist-two polarized operator matrix elements $A_{gg,Q}^{(3)}$ and $A_{Qq}^{(3),PS}$ as functions of the heavy quark mass ratio. We discuss the mathematical structure of these objects and discuss their phenomenological importance for the variable flavour number scheme and mathematical and computer-algebraic aspects of their calculation. We further address the impact of the heavy quarks to the scheme-invariant evolution of structure functions and introduce a Fortran library for their evaluation. We also discuss a computer algebra implementation of a solver for partial linear difference equations.

==> input/pol-OMEs/AgqQpol.tex <==
\begin{eqnarray}
A_{gq,Q} &=&
	a_s ^2  \textcolor{blue}{C_F T_F} \Biggl\{
        \frac{8  L_M ^2 (2+N)}{3 N (1+N)}
        +\frac{8 (2+N) \big(
                22+41 N+28 N^2\big)}{27 N (1+N)^3}
\nonumber\\&&		
        + L_M  \biggl[
                \frac{16 (2+N) (2+5 N)}{9 N (1+N)^2}
                -\frac{16 (2+N) S_1}{3 N (1+N)}
        \biggr]
        -\frac{8 (2+N) (2+5 N)}{9 N (1+N)^2} S_1
        +\frac{4 (2+N) S_1^2}{3 N (1+N)}
\nonumber\\&&	
        +\frac{4 (2+N) S_2}{3 N (1+N)}
	\Biggr\}
+ a_s ^3 \Biggl\{
	 \textcolor{blue}{C_F T_F^2} \biggl\{
                \frac{992  L_M  (2+N)}{27 N (1+N)}
                +\frac{64  L_M ^3 (2+N)}{9 N (1+N)}
\nonumber\\&&		
                -\frac{32 (2+N) \big(
                        98+369 N+408 N^2+164 N^3\big)}{81 N (1+N)^4}
                + L_M ^2 \biggl[
                        \frac{32 (2+N) (2+5 N)}{9 N (1+N)^2}
\nonumber\\&&			
                        -\frac{32 (2+N) S_1}{3 N (1+N)}
                \biggr]
                +\biggl[
                        \frac{32 (2+N) \big(
                                22+41 N+28 N^2\big)}{27 N (1+N)^3}
                        +\frac{16 (2+N) S_2}{3 N (1+N)}
                \biggr] S_1
\nonumber\\&&		
                -\frac{16 (2+N) (2+5 N)}{9 N (1+N)^2} S_1^2
                +\frac{16 (2+N) S_1^3}{9 N (1+N)}
                -\frac{16 (2+N) (2+5 N)}{9 N (1+N)^2} S_2
                +\frac{32 (2+N) S_3}{9 N (1+N)}
\nonumber\\&&		
                +\biggl[
                        -\frac{32 (2+N) (2+5 N)}{9 N (1+N)^2}
                        +\frac{32 (2+N) S_1}{3 N (1+N)}
                \biggr] \zeta_2
                -\frac{64 (2+N) \zeta_3}{9 N (1+N)}
	\biggr\}
\nonumber\\&&	
	+ \textcolor{blue}{C_F N_F T_F^2} \biggl\{
                \frac{32  L_M 
                ^3 (2+N)}{9 N (1+N)}
                -
                \frac{32 (2+N) \big(
                        98+369 N+408 N^2+164 N^3\big)}{81 N (1+N)^4}
\nonumber\\&&			
                + L_M  \biggl[
                        \frac{32 (2+N) \big(
                                40+83 N+34 N^2\big)}{27 N (1+N)^3}
                        +\frac{32 (2+N) (2+5 N)}{9 N (1+N)^2} S_1
                        -\frac{16 (2+N) S_1^2}{3 N (1+N)}
\nonumber\\&&			
                        -\frac{16 (2+N) S_2}{3 N (1+N)}
                \biggr]
                +\biggl[
                        \frac{32 (2+N) \big(
                                22+41 N+28 N^2\big)}{27 N (1+N)^3}
                        +\frac{16 (2+N) S_2}{3 N (1+N)}
                \biggr] S_1
\nonumber\\&&		
                -\frac{16 (2+N) (2+5 N)}{9 N (1+N)^2} S_1^2
                +\frac{16 (2+N) S_1^3}{9 N (1+N)}
                -\frac{16 (2+N) (2+5 N)}{9 N (1+N)^2} S_2
                +\frac{32 (2+N) S_3}{9 N (1+N)}
\nonumber\\&&		
                +\biggl[
                        -\frac{16 (2+N) (2+5 N)}{9 N (1+N)^2}
                        +\frac{16 (2+N) S_1}{3 N (1+N)}
                \biggr] \zeta_2
                -\frac{32 (2+N) \zeta_3}{9 N (1+N)}
	\biggr\}
\nonumber\\&&	
	+ \textcolor{blue}{C_A C_F T_F} \biggl\{
                \frac{4 (2+N) P_{127}}{81 N^5 (1+N)^5}
                + L_M ^3 \biggl[
                        -\frac{8 (2+N) \big(
                                4+11 N+11 N^2\big)}{9 N^2 (1+N)^2}
                        +\frac{16 (2+N) S_1}{9 N (1+N)}
                \biggr]
\nonumber\\&&		
                + L_M ^2 \biggl[
                        \frac{4 P_{123}}{9 N^3 (1+N)^3}
                        +\frac{16 \big(
                                6-8 N+9 N^2+5 N^3\big)}{9 N^2 
(1+N)^2} S_1
                        -\frac{8 (2+N) S_1^2}{3 N (1+N)}
                        -\frac{8 (2+N) S_2}{N (1+N)}
\nonumber\\&&			
                        -\frac{16 (2+N) S_{-2}
                        }{N (1+N)}
                \biggr]
                + L_M  \Biggl[
                        -
                        \frac{8 P_{126}}{27 (-1+N) N^4 (1+N)^4}
                        +\biggl[
                                -\frac{8 P_{124}}{27 N^3 (1+N)^3}
\nonumber\\&&				
                                +\frac{56 (2+N) S_2}{3 N (1+N)}
                        \biggr] S_1
                        +\frac{4 \big(
                                -12+110 N+63 N^2+13 N^3\big)}{9 N^2 
(1+N)^2} S_1^2
                        +\frac{8 (2+N) S_1^3}{9 N (1+N)}
\nonumber\\&&			
                        -\frac{4 \big(
                                20-2 N+15 N^2+9 N^3\big)}{3 N^2 
(1+N)^2} S_2
                        +\frac{256 (2+N) S_3}{9 N (1+N)}
                        +\biggl[
                                -\frac{32 P_{114}}{3 (-1+N) N^2 
(1+N)^2}
\nonumber\\&&
                                +\frac{128 (2+N) S_1}{3 N (1+N)}
                        \biggr] S_{-2}
                        +\frac{64 (2+N) S_{-3}}{3 N (1+N)}
                        -\frac{64 (2+N) S_{-2,1}}{3 N (1+N)}
                        +\frac{64 (2+N) \zeta_3}{N (1+N)}
                \Biggr]
\nonumber\\&&		
                +\biggl[
                        -\frac{8 (2+N) P_{121}}{81 N^2 (1+N)^4}
                        -\frac{4 (2+N) \big(
                                24+41 N+53 N^2\big)}{9 N^2 (1+N)^2} S_2
                        +\frac{32 (2+N) S_3}{9 N (1+N)}
                \biggr] S_1
\nonumber\\&&		
                +\biggl[
                        \frac{4 (2+N) \big(
                                48+371 N+568 N^2+389 N^3\big)}{27 N^2 
(1+N)^3}
                        +\frac{16 (2+N) S_2}{3 N (1+N)}
                \biggr] S_1^2
\nonumber\\&&		
                -\frac{4 (2+N) \big(
                        8+19 N+31 N^2\big)}{9 N^2 (1+N)^2} S_1^3
                +\frac{16 (2+N) S_1^4}{9 N (1+N)}
\nonumber\\&&		
                +\frac{4 (2+N) \big(
                        16+59 N+68 N^2+49 N^3\big)}{9 N^2 (1+N)^3} 
S_2
                -\frac{8 (2+N) \big(
                        8+11 N+11 N^2\big)}{9 N^2 (1+N)^2} S_3
\nonumber\\&&			
                +\biggl[
                        \frac{4 P_{122}
                        }{9 N^3 (1+N)^3}
                        -
                        \frac{4 \big(
                                60+70 N+135 N^2+53 N^3\big)}{9 N^2 
(1+N)^2} S_1
                        +\frac{20 (2+N) S_1^2}{3 N (1+N)}
                        +\frac{4 (2+N) S_2}{N (1+N)}
\nonumber\\&&			
                        +\frac{8 (2+N) S_{-2}}{N (1+N)}
                \biggr] \zeta_2
                +\biggl[
                        \frac{8 (2+N) \big(
                                4+11 N+11 N^2\big)}{9 N^2 (1+N)^2}
                        -\frac{16 (2+N) S_1}{9 N (1+N)}
                \biggr] \zeta_3
	\biggr\}
\nonumber\\&&	
	+ \textcolor{blue}{C_F^2 T_F}  \biggl\{
                -\frac{8 (2+N) S_3 P_{115}}{9 N^3 (1+N)^3}
                +\frac{4 (2+N) S_2 P_{125}}{27 N^4 (1+N)^4}
                +\frac{(2+N) P_{129}}{162 N^5 (1+N)^6}
\nonumber\\&&		
                + L_M ^3 \biggl[
                        \frac{4 (2+N) \big(
                                6+N+N^2
                        \big)
\big(-4+3 N+3 N^2\big)}{9 N^3 (1+N)^3}
                        -\frac{16 (2+N) S_1}{9 N (1+N)}
                \biggr]
\nonumber\\&&		
                + L_M ^2 \biggl[
                        -\frac{2 (2+N) P_{117}}{9 N^3 (1+N)^3}
                        +\frac{16 (2+N) (-3+4 N)}{9 N^2 (1+N)} S_1
                        +\frac{8 (2+N) S_1^2}{3 N (1+N)}
                        -\frac{40 (2+N) S_2}{3 N (1+N)}
                \biggr]
\nonumber\\&&		
                + L_M  \Biggl[
                        -\frac{4 (2+N) S_2 P_{118}}{9 N^3 (1+N)^3}
                        -\frac{2 P_{128}}{27 (-1+N) N^5 (1+N)^4}
                        +\biggl[
                                \frac{8 (2+N) P_{116}}{27 N^3 
(1+N)^3}
\nonumber\\&&
                                +\frac{88 (2+N) S_2}{3 N (1+N)}
                        \biggr] S_1
                        -\frac{4 (2+N) \big(
                                -12+7 N+25 N^2\big)}{9 N^2 (1+N)^2} 
S_1^2
                        -\frac{8 (2+N) S_1^3}{9 N (1+N)}
\nonumber\\&&			
                        +\frac{176 (2+N) S_3}{9 N (1+N)}
                        +\frac{128 S_{-2}}{(-1+N) N^2 (1+N)^2}
                        -\frac{32 (2+N) S_{2,1}}{3 N (1+N)}
                        -\frac{64 (2+N) \zeta_3}{N (1+N)}
                \Biggr]
\nonumber\\&&		
                +\biggl[
                        \frac{8 (2+N) P_{120}}{81 N^2 (1+N)^4}
                        +\frac{4 (2+N) \big(
                                6+17 N+29 N^2\big)}{9 N^2 (1+N)^2} 
S_2
                        -\frac{32 (2+N) S_3}{9 N (1+N)}
                \biggr] S_1
\nonumber\\&&		
                +\biggl[
                        -\frac{4 (2+N) \big(
                                12+116 N+175 N^2+161 N^3\big)}{27 N^2 
(1+N)^3}
                        -\frac{16 (2+N) S_2}{3 N (1+N)}
                \biggr] S_1^2
\nonumber\\&&		
                +\frac{4 (2+N) \big(
                        2+11 N+23 N^2\big)}{9 N^2 (1+N)^2} S_1^3
                -\frac{16 (2+N) S_1^4}{9 N (1+N)}
                +\frac{16 (2+N) S_4}{3 N (1+N)}
                +\biggl[
                        \frac{2 (2+N) P_{119}}{9 N^3 (1+N)^3}
\nonumber\\&&			
                        +\frac{4 (2+N) \big(
                                12+5 N+11 N^2\big)}{9 N^2 (1+N)^2} 
S_1
                        -\frac{20 (2+N) S_1^2}{3 N (1+N)}
                        +\frac{28 (2+N) S_2}{3 N (1+N)}
                \biggr] \zeta_2
\nonumber\\&&		
                +\biggl[
                        -\frac{4 (2+N) \big(
                                6+N+N^2
                        \big)
\big(-4+3 N+3 N^2\big)}{9 N^3 (1+N)^3}
                        +\frac{16 (2+N) S_1}{9 N (1+N)}
                \biggr] \zeta_3
	\biggr\}
+ a_{gq,Q}^{(3)}
	\Biggr\}
\end{eqnarray}

\begin{eqnarray}
P_{114} &=& 5 N^4+9 N^3-4 N^2-4 N+6, \\
P_{115} &=& 7 N^4+14 N^3+23 N^2+16 N-36, \\
P_{116} &=& 23 N^4-149 N^3-88 N^2-6 N-36, \\
P_{117} &=& 69 N^4+66 N^3+43 N^2+46 N+96, \\
P_{118} &=& 145 N^4+248 N^3+79 N^2-24 N+72, \\
P_{119} &=& 204 N^4+390 N^3+187 N^2+37 N+114, \\
P_{120} &=& 472 N^4+1269 N^3+1551 N^2+724 N+132, \\
P_{121} &=& 1252 N^4+2997 N^3+3360 N^2+1819 N+528, \\
P_{122} &=& 7 N^5-5 N^4-9 N^3+29 N^2-100 N-12, \\
P_{123} &=& 69 N^5+276 N^4+263 N^3+12 N^2+172 N+48, \\
P_{124} &=& 197 N^5+791 N^4+952 N^3+148 N^2+348 N+144, \\
P_{125} &=& 175 N^6+552 N^5+657 N^4+376 N^3+204 N^2+540 N+216, \\
P_{126} &=& 8 N^8+341 N^7+1276 N^6+617 N^5-1835 N^4+44 N^3
\nonumber\\&&
+1037 N^2+204 N+36, \\
P_{127} &=& 3347 N^8+11540 N^7+16090 N^6+10202 N^5+3200 N^4
\nonumber\\&&
+430 N^3+3 N^2+36 N+108, \\
P_{128} &=& 51 N^9-300 N^8-674 N^7-360 N^6-1775 N^5+456 N^4
\nonumber\\&&
-662 N^3-4296 N^2-216 N+864, \\
P_{129} &=& 2067 N^9+12639 N^8+23134 N^7+12958 N^6+2319 N^5
\nonumber\\&&
+691 N^4+448 N^3+23136 N^2+15840 N+4752
\end{eqnarray}

